Kuroda's Translation for the $\lambda\Pi$-Calculus Modulo Theory and Dedukti

Kuroda's translation embeds classical first-order logic into intuitionistic logic, through the insertion of double negations. Recently, Brown and Rizkallah extended this translation to higher-order logic. In this paper, we adapt it for theories encoded in higher-order logic in the lambdaPi-calculus modulo theory, a logical framework that extends lambda-calculus with dependent types and user-defined rewrite rules. We develop a tool that implements Kuroda's translation for proofs written in Dedukti, a proof language based on the lambdaPi-calculus modulo theory.

==> eptcsdata.tex <==
\providecommand{\firstpage}{35}
\providecommand{\publicationstatus}{Rabe, Sacerdoti Coen (Eds): LFMTP 2024\\
EPTCS 404, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.404.3}{10.4204/EPTCS.404.3}}

